Higher tensor network states in two spatial dimensions: fundamental theorem for open boundary conditions

We introduce a class of two-dimensional tensor network states obtained by categorifying matrix product states. This procedure leads us to consider bond spaces provided by a 2-vector space associated with the 2-cells of the underlying lattice. Tensor network representations are then defined as module categories over the free monoidal category on a monoidal signature encoding the lattice geometry. We prove a fundamental theorem stating that two representations generating the same states with suitable open boundary conditions are equivalent as module categories. Finally, we introduce a notion of 2-injectivity, a categorified analogue of the injectivity condition for matrix product states.

==> tikz.tex <==
\pgfdeclarelayer{back}
\pgfdeclarelayer{front}
\pgfsetlayers{back,main,front}

\def\fixboundingbox{
    \path [use as bounding box] (current bounding box.south west) rectangle (current bounding box.north east);
}

\def\ExtractBase#1#2\endExtract{\def\Mbase{#1}}
\def\ExtractBaseB#1#2\endExtract{\def\MbaseB{#1}}

\tikzset{->-/.style={
        decoration={
            markings,
            mark=at position #1 with {
                \pgftransformxshift{2.5pt}
                \arrow{Triangle[width=3.5pt, length=3.5pt]}
            }
        },
        postaction={decorate}
    }
}

\tikzset{-<-/.style={
        decoration={
            markings,
            mark=at position #1 with {
                \pgftransformxshift{-2.5pt}
                \arrowreversed{Triangle[width=3.5pt, length=3.5pt]}
            }
        },
        postaction={decorate}
    }
}

\tikzset{
    every picture/.append style={
        line join=round,
        line width = 0.7pt,
        line cap=round
    }
}

\tikzset{
    mathpoly/.style={
        baseline=0ex,        
        x=1.3ex, y=1.3ex,      
        line width=0.11ex,      
        line join=round        
    }
}

\tikzset{mpoint/.style={ transform shape, sloped, 
minimum width=20pt, minimum height=4pt, inner sep=0pt, ultra thin, font=\tiny}}

\tikzset{
    clip even odd rule/.code={\pgfseteorule},
    invclip/.style={
        clip,
        insert path=[clip even odd rule]{
            [reset cm](-20cm,-20cm) rectangle (20cm,20cm)
        }
    }
}
  
\newcommand\clipIntersection[1]{
    (#1.north west) -- (#1.north east) -- (#1.south east) -- (#1.south west) -- (#1.north west)
}

\tikzset{every label/.style={label distance=-1pt}}

% ------------------------------------------------------

\tikzstyle{dot}=[dash pattern= on 0.6pt off 2.1pt]
\tikzstyle{mor}=[circle, minimum size=4pt, inner sep=0pt, fill=black]
\tikzstyle{ten}=[circle, minimum size=5pt, inner sep=0pt, fill=gray!20, draw]
\tikzset{gmor/.style={mor, draw=none, fill=none, overlay}}
\tikzset{gten/.style={ten, draw=none, fill=none, overlay}}
\tikzset{fake/.style={inner sep=0pt, outer sep=0pt, minimum size=0pt, draw=none, fill=none}}
\tikzset{leg/.style={inner sep=0pt, draw=none, fill=none}}
\tikzstyle{obj}=[draw=black]


% ------------------------------------------------------

\newcommand\clipAroundNodes[2]{
    \begin{pgfscope}
        \begin{scope}[overlay]
            \path[invclip] \foreach \n in {#1} { \clipIntersection{\n} };
            #2
        \end{scope}
    \end{pgfscope}
}

% ------------------------------------------------------
% ------------------------------------------------------

\newsavebox{\msquarebox}

\sbox{\msquarebox}{\tikz[mathpoly, baseline=0ex] \draw[scale=1, shift={(0, 0.5)}] (-0.5, -0.5) rectangle (0.5, 0.5);}

\newcommand{\msquare}{\mathord{\mathchoice{\usebox{\msquarebox}}{\usebox{\msquarebox}}{\scalebox{0.8}{\usebox{\msquarebox}}}{\scalebox{0.6}{\usebox{\msquarebox}}}}}

\newsavebox{\mhexagonbox}

\sbox{\mhexagonbox}{\tikz[mathpoly] \draw[scale=1, shift={(0, 1/2)}] 
            ({-120}:{1/(2*cos(30))}) 
             -- ({-60}:{1/(2*cos(30))}) 
             -- ({0}:{1/(2*cos(30))}) 
             -- ({60}:{1/(2*cos(30))}) 
             -- ({120}:{1/(2*cos(30))}) 
             -- ({180}:{1/(2*cos(30))}) 
             -- cycle;
}

\newcommand{\mhexagon}{\mathord{\mathchoice{\usebox{\mhexagonbox}}{\usebox{\mhexagonbox}}{\scalebox{0.8}{\usebox{\mhexagonbox}}}{\scalebox{0.6}{\usebox{\mhexagonbox}}}}}


% ------------------------------------------------------
% ------------------------------------------------------

\newcommand{\MPS}[2]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \node[fake] (w) at (-\l,0) {};
        \node[fake] (e) at (\l,0) {};
        \node[leg,label={[label distance=-1pt]above:{${\sss #2}$}}] (t) at (0,.6*\l) {};
        \node[ten,label={[label distance=-1pt]below:{${\sss #1}$}}] (n) at (0,0) {};
        \draw[obj,->-=.55] (e) -- (n);
        \draw[obj,->-=.55] (n) -- (w);
        \draw[obj] (t) -- (n);
    \end{tikzpicture}
}

\newcommand{\MPSthree}[4][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \node[ten,label=left:{${\sss \phi^{#1}}$}] (phi) at (0,0) {};
        \node[ten,label=right:{${\sss v^{#1}}$}] (v) at (4*\l,0) {};
        \node[leg,label={[label distance=-1pt]above:{${\sss #2}$}}] (t1) at (\l,.6*\l) {};
        \node[leg,label={[label distance=-1pt]above:{${\sss #3}$}}] (t2) at (2*\l,.6*\l) {};
        \node[leg,label={[label distance=-1pt]above:{${\sss #4}$}}] (t3) at (3*\l,.6*\l) {};
        \node[ten,label={[label distance=-1pt]below:{${\sss #1}$}}] (n1) at (\l,0) {};
        \node[ten,label={[label distance=-1pt]below:{${\sss #1}$}}] (n2) at (2*\l,0) {};
        \node[ten,label={[label distance=-1pt]below:{${\sss #1}$}}] (n3) at (3*\l,0) {};
        \draw[obj,->-=.55] (v) -- (n3);
        \draw[obj,->-=.55] (n3) -- (n2);
        \draw[obj,->-=.55] (n2) -- (n1);
        \draw[obj,->-=.55] (n1) -- (phi);
        \draw[obj] (t1) -- (n1);
        \draw[obj] (t2) -- (n2);
        \draw[obj] (t3) -- (n3);
    \end{tikzpicture}
}

\newcommand{\MPSQ}[3][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \node[leg,label={[label distance=-1pt]above:{${\sss #2}$}}] (t) at (0,.6*\l) {};
        \node[ten,label={[label distance=-1pt]below:{${\sss #1}$}}] (n) at (0,0) {};
        \ifthenelse{\equal{#3}{l}}{
            \node[fake] (w) at (-2*\l,0) {};
            \node[fake] (e) at (\l,0) {};
            \node[ten,label={[label distance=-1pt]below:{${\sss Q}$}}] (q) at (-\l,0) {};
            \draw[obj,->-=.55] (e) -- (n);
            \draw[obj,->-=.55] (n) -- (q);
            \draw[obj,->-=.55] (q) -- (w);
        }{
            \node[fake] (w) at (-\l,0) {};
            \node[fake] (e) at (2*\l,0) {};
            \node[ten,label={[label distance=-1pt]below:{${\sss Q}$}}] (q) at (\l,0) {};
            \draw[obj,->-=.55] (e) -- (q);
            \draw[obj,->-=.55] (q) -- (n);
            \draw[obj,->-=.55] (n) -- (w);
        }
        \draw[obj] (t) -- (n);
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcommand{\stringDiag}[1]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]current bounding box.center)}, every label/.style={label distance=-5pt}]    
    \def\l{1};
    \def\ll{1};
    \ifthenelse{#1=1}{
        \foreach \x/\n in {1/1,2/1,3/1,4/2,5/1,6/2,7/2}{
            \node[gmor,label=below:{${\sss X_\n}$}] (g1\x) at (\x*\l-.5*\l,-.5*\ll) {};
        }
        \foreach \x/\n in {1/2,2/1,3/2,4/1,5/2,6/1,7/1}{
            \node[gmor,label=above:{${\sss X_\n}$}] (g3\x) at (\x*\l-.5*\l,2.5*\ll) {};
        }
        \foreach \x/\y/\n in {3/0/3,5/0/6,2/1/2,4/1/5,6/1/8,1/2/1,3/2/4,5/2/7}{
            \node[mor, label={[label distance=-1pt]left:{${\sss f_{i_{\n}}}$}}] (n\n) at (\x*\l,\y*\ll) {};
        }
        \draw[obj] (g11) -- ($(g11)+(0,2*\ll)$) -- (g32);
        \draw[obj] (g12) -- ($(g12)+(0,\ll)$) -- (g34);
        \draw[obj] (g13) -- (g36);
        \draw[obj] (g14) -- (g31);
        \draw[obj] (g15) -- ($(g17)+(0,2*\ll)$) -- (g37);
        \draw[obj] (g16) -- (g33);
        \draw[obj] (g17) -- ($(g17)+(0,\ll)$) -- (g35);
    }{}
    \ifthenelse{#1=2}{
        \node[gmor,label=below:{${\sss X_1}$}] (g11) at (0,-\l/2) {};
        \node[gmor,label=below:{${\sss X_1}$}] (g12) at (\l,-\l/2) {};
        \node[gmor,label=below:{${\sss X_1}$}] (g13) at (2*\l,-\l/2) {};
        \node[gmor,label=left:{${\sss X_2}$}] (g20) at (-\l/2,0) {};
        \node[gmor,label=right:{${\sss X_2}$}] (g24) at (2.5*\l,0) {};
        \node[gmor,label=above:{${\sss X_1}$}] (g31) at (0,\l/2) {};
        \node[gmor,label=below:{${\sss X_1}$}] (g35) at (3*\l,\l/2) {};
        \node[gmor,label=left:{${\sss X_2}$}] (g41) at (\l/2,\l) {};
        \node[gmor,label=right:{${\sss X_2}$}] (g46) at (3.5*\l,\l) {};
        \node[gmor,label=above:{${\sss X_1}$}] (g52) at (\l,1.5*\l) {};
        \node[gmor,label=left:{${\sss X_2}$}] (g62) at (1.5*\l,2*\l) {};
        \node[gmor,label=right:{${\sss X_2}$}] (g66) at (3.5*\l,2*\l) {};
        \node[gmor,label=above:{${\sss X_1}$}] (g73) at (2*\l,2.5*\l) {};
        \node[gmor,label=above:{${\sss X_1}$}] (g75) at (3*\l,2.5*\l) {};
        \draw[obj] (g20) -- (g24);
        \draw[obj] (g41) -- (g46);
        \draw[obj] (g62) -- (g66);
        \draw[obj] (g11) -- (g31);
        \draw[obj] (g12) -- (g52);
        \draw[obj] (g13) -- (g73);
        \draw[obj] (g35) -- (g75);
        \foreach \x/\y/\n in {0/0/1,1/0/2,2/0/3,1/1/4,2/1/5,3/1/6,2/2/7,3/2/8}{
        \node[mor,label=below left:{${\sss f_{i_{\n}}}$}] () at (\x*\l,\y*\l) {};
    }
    }{}
    \end{tikzpicture}
}

\newcommand{\young}[1]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,1.35)}]
    \def\l{.9};
    \ifthenelse{#1=1}{
        \path[pattern=north east lines, rounded corners=4pt, line width=.4pt, pattern color=black!60] 
        (0,\l) -- (\l,\l) -- (\l,2*\l) -- (2*\l,2*\l) -- (2*\l,3*\l) -- (0,3*\l) --cycle;
        \draw[obj] (0,0) -- (3*\l,0) -- (3*\l,\l) -- (4*\l,\l) -- (4*\l,3*\l) -- (0,3*\l) --cycle;
        \draw[obj] (\l,0) -- (\l,3*\l);
        \draw[obj] (2*\l,0) -- (2*\l,3*\l);
        \draw[obj] (0,\l) -- (3*\l,\l);
        \draw[obj] (0,2*\l) -- (4*\l,2*\l);
        \draw[obj] (3*\l,\l) -- (3*\l,3*\l);
    }{}
    \ifthenelse{#1=2}{
        \draw[obj] (0,0) -- (3*\l,0) -- (3*\l,\l) -- (4*\l,\l) -- (4*\l,3*\l) -- (2*\l,3*\l) -- (2*\l,2*\l) -- (\l,2*\l) -- (\l,\l) -- (0,\l) --cycle;
        \draw[obj] (\l,0) -- (\l,\l);
        \draw[obj] (2*\l,0) -- (2*\l,2*\l);
        \draw[obj] (\l,\l) -- (3*\l,\l);
        \draw[obj] (2*\l,2*\l) -- (4*\l,2*\l);
        \draw[obj] (3*\l,\l) -- (3*\l,3*\l);
    }{}
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcommand{\TLine}[5]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
    \def\l{.75}
    \fill[color=LimeGreen!20] (-\l,-\l) rectangle (\l,\l);
    \node[fake] (r) at (\l,0) {};
    \node[fake] (l) at (-\l,0) {};
    \ifthenelse{\equal{#4}{}}{}{
        \node[ten,label=right:{${\sss #4}$}] (r) at (r) {};
    }
    \ifthenelse{\equal{#5}{}}{}{
        \node[ten,label=left:{${\sss #5}$}] (l) at (l) {};
    }
    \draw[obj,->-=.5] (r) -- (l);
    \ifthenelse{\equal{#1}{}}{}{
        \node[mlabel, anchor=north] at (0,-.1*\l) {${\sss #1}$};
    }
    \ifthenelse{\equal{#2}{}}{}{
        \node[mlabel, anchor=north east] at (\l,\l) {${\sss #2}$};
    }
    \ifthenelse{\equal{#3}{}}{}{
        \node[mlabel, anchor=south east] at (\l,-\l) {${\sss #3}$};
    }
    \end{tikzpicture}
}

\newcommand{\TTLine}[9]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]c)}, mlabel/.style={inner sep=1pt}]
        \def\l{.75}
        \coordinate (c) at (0,.5*\l);
        \fill[color=LimeGreen!20] (-\l,-\l) rectangle (\l,2*\l);
        \node[fake] (r1) at (\l,0) {};
        \node[fake] (l1) at (-\l,0) {};
        \node[fake] (r2) at (\l,\l) {};
        \node[fake] (l2) at (-\l,\l) {};
        \ifthenelse{\equal{#6}{}}{}{
            \node[ten,label=right:{${\sss #6}$}] (r1) at (r1) {};
        }
        \ifthenelse{\equal{#7}{}}{}{
            \node[ten,label=right:{${\sss #7}$}] (r2) at (r2) {};
        }
        \ifthenelse{\equal{#8}{}}{}{
            \node[ten,label=left:{${\sss #8}$}] (l1) at (l1) {};
        }
        \ifthenelse{\equal{#9}{}}{}{
            \node[ten,label=left:{${\sss #9}$}] (l2) at (l2) {};
        }
        \draw[obj,->-=.5] (r1) -- (l1);
        \draw[obj,->-=.5] (r2) -- (l2);
        \ifthenelse{\equal{#1}{}}{}{
            \node[mlabel, anchor=north] at (0,-.1*\l) {${\sss #1}$};
        }
        \ifthenelse{\equal{#2}{}}{}{
            \node[mlabel, anchor=north] at (0,.9*\l) {${\sss #2}$};
        }
        \ifthenelse{\equal{#3}{}}{}{
            \node[mlabel, anchor=north east] at (\l,2*\l) {${\sss #3}$};
        }
        \ifthenelse{\equal{#4}{}}{}{
            \node[mlabel, anchor=east] at (\l,.5*\l) {${\sss #4}$};
        }
        \ifthenelse{\equal{#5}{}}{}{
            \node[mlabel, anchor=south east] at (\l,-\l) {${\sss #5}$};
        }
    \end{tikzpicture}
}

\newcommand{\NatLine}[5]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
    \def\l{.75}
    \fill[color=LimeGreen!20] (-\l,-\l) rectangle (\l,\l);
    \node[fake] (r) at (\l,0) {};
    \node[fake] (l) at (-\l,0) {};
    \ifthenelse{\equal{#5}{}}{
        \node[ten] (n) at (0,0) {};
    }{
        \node[ten,label=below:{${\sss #5}$}] (n) at (0,0) {};
    }
    \draw[obj,->-=.5] (r) -- (n);
    \draw[obj,->-=.5] (n) -- (l);
    \ifthenelse{\equal{#1}{}}{}{
        \node[mlabel, anchor=south] at (.5*\l,.1*\l) {${\sss #1}$};
    }
    \ifthenelse{\equal{#2}{}}{}{
        \node[mlabel, anchor=south] at (-.5*\l,.1*\l) {${\sss #2}$};
    }
    \ifthenelse{\equal{#3}{}}{}{
        \node[mlabel, anchor=north east] at (\l,\l) {${\sss #3}$};
        \node[mlabel, anchor=north west] at (-\l,\l) {${\sss #3}$};
    }
    \ifthenelse{\equal{#4}{}}{}{
        \node[mlabel, anchor=south east] at (\l,-\l) {${\sss #4}$};
        \node[mlabel, anchor=south west] at (-\l,-\l) {${\sss #4}$};
    }
    \end{tikzpicture}
}

\newcommand{\NatCoup}[7]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
    \def\l{.75}
    \fill[color=LimeGreen!20] (-\l,-1.5*\l) rectangle (\l,1.5*\l);
    \node[fake] (ru) at (\l,.5*\l) {};
    \node[fake] (rd) at (\l,-.5*\l) {};
    \node[fake] (l) at (-\l,0) {};
    \ifthenelse{\equal{#7}{}}{
        \node[ten] (n) at (0,0) {};
    }{
        \node[ten,label=below:{${\sss #7 \;}$}] (n) at (0,0) {};
    }
    \draw[obj,->-=.35,rounded corners=.2*\l*1cm] (ru) -- (.35*\l,.5*\l) -- (n);
    \draw[obj,->-=.35,rounded corners=.2*\l*1cm] (rd) -- (.35*\l,-.5*\l) -- (n);
    \draw[obj,->-=.5] (n) -- (l);
    \ifthenelse{\equal{#1}{}}{}{
        \node[mlabel, anchor=north] at (.6*\l,-.6*\l) {${\sss #1}$};
    }
    \ifthenelse{\equal{#2}{}}{}{
        \node[mlabel, anchor=south] at (.6*\l,.6*\l) {${\sss #2}$};
    }
    \ifthenelse{\equal{#3}{}}{}{
        \node[mlabel, anchor=south] at (-.5*\l,.1*\l) {${\sss #3}$};
    }
    \ifthenelse{\equal{#4}{}}{}{
        \node[mlabel, anchor=north west] at (-\l,1.5*\l) {${\sss #4}$};
    }
    \ifthenelse{\equal{#5}{}}{}{
        \node[mlabel, anchor=east] at (\l,0) {${\sss #5}$};
    }
    \ifthenelse{\equal{#6}{}}{}{
        \node[mlabel, anchor=south west] at (-\l,-1.5*\l) {${\sss #6}$};
    }
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcommand{\PEPSSKEW}[3]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]base)}, mlabel/.style={inner sep=1pt}]
    \def\l{.75}
    \coordinate (base) at (0,2*\l);
    \ifthenelse{\equal{#2}{B}}{\def\cMain{CornflowerBlue!20}}{\def\cMain{LimeGreen!20}}
    
    \ifthenelse{#1=0}{}{
        \fill[color=\cMain] (-\l,-\l) -- (5*\l,-\l) -- (5*\l,\l) -- (7*\l,\l) -- (7*\l,5*\l) -- (3*\l,5*\l) -- (3*\l,3*\l) -- (\l,3*\l) -- (\l,\l) -- (-\l,\l) -- cycle;
    }
    
    \foreach \n/\x/\y in {1/0/0, 2/2/0, 3/4/0, 4/2/2, 5/4/2, 6/6/2, 7/4/4, 8/6/4}{
        \ifthenelse{#3=0}{
            \node[fake] (f\n) at (\x*\l-.25*\l, \y*\l+.25*\l) {};
        }{
        \node[leg,label={[label distance=-6pt]above left:{${\sss i_{\n}}$}}] (f\n) at (\x*\l-.25*\l, \y*\l+.25*\l) {};
        }
        \node[ten,label={[label distance=-3pt]below left:{${\sss #2}$}}] (c\n) at (\x*\l, \y*\l) {};
        \draw[obj] (c\n) -- (f\n);
    }
    
    \foreach \n/\x/\y in {1/0/0, 2/2/0, 3/4/0, 6/6/2}{
        \node[ten,label=below:{${\sss v^{#2}_1}$}] (b\n) at (\x*\l, \y*\l-\l) {};
        \draw[obj,->-=.5] (b\n) -- (c\n);
    }
    \foreach \n/\x/\y in {3/4/0, 6/6/2, 8/6/4}{
        \node[ten,label=right:{${\sss v^{#2}_2}$}] (r\n) at (\x*\l+\l, \y*\l) {};
        \draw[obj,->-=.5] (r\n) -- (c\n);
    }
    
    \foreach \n/\x/\y in {1/0/0, 4/2/2, 7/4/4, 8/6/4}{
        \node[ten,label=above:{${\sss \phi^{#2}_1}$}] (t\n) at (\x*\l, \y*\l+\l) {};
        \draw[obj,->-=.5] (c\n) -- (t\n);
    }
    \foreach \n/\x/\y in {1/0/0, 4/2/2, 7/4/4}{
        \node[ten,label=left:{${\sss \phi^{#2}_2}$}] (l\n) at (\x*\l-\l, \y*\l) {};
        \draw[obj,->-=.5] (c\n) -- (l\n);
    }
    
    \foreach \a/\b in {2/1, 3/2, 5/4, 6/5, 8/7, 2/4, 3/5, 5/7, 6/8}{
        \draw[obj,->-=.5] (c\a) -- (c\b);
    }
    \end{tikzpicture}
}

% ------------------------------------------------------

\newboolean{pepsQL}
\newboolean{pepsQR}
\newboolean{pepsQT}
\newboolean{pepsQB}

\def\pepsSplit#1#2#3#4#5#6\pepsEnd{
    \def\pepsBase{#1}\def\pepsLi{#2}\def\pepsLii{#3}\def\pepsLiii{#4}\def\pepsLiv{#5}}

\newcommand{\pepsCornerLabel}[7]{
    \ifthenelse{\equal{#1}{-}}{}{
        \ifthenelse{\boolean{#2}}{
            \node[mlabel, anchor=#6] at (#4.5*\l, #5\l) {${\sss \Mbase_{#1}}$};
        }{
        \ifthenelse{\boolean{#3}}{
            \node[mlabel, anchor=#7] at (#4\l, #5.5*\l) {${\sss \Mbase_{#1}}$};
        }{
            \node[mlabel, anchor=#6 #7] at (#4\l, #5\l) {${\sss \Mbase_{#1}}$};
        }
        }
    }
}

    \newcommand{\PEPS}[9]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
    \def\l{.75}
    
    \ifthenelse{\equal{#2}{B}}{
        \def\cMain{CornflowerBlue!20}
        \def\cQ{LimeGreen!20}
    }{
        \def\cMain{LimeGreen!20}
        \def\cQ{CornflowerBlue!20}
    }
    
    \ifthenelse{\equal{#8}{Q}}{\setboolean{pepsQL}{true}}{\setboolean{pepsQL}{false}}
    \ifthenelse{\equal{#7}{Q}}{\setboolean{pepsQR}{true}}{\setboolean{pepsQR}{false}}
    \ifthenelse{\equal{#9}{Q}}{\setboolean{pepsQT}{true}}{\setboolean{pepsQT}{false}}
    \ifthenelse{\equal{#6}{Q}}{\setboolean{pepsQB}{true}}{\setboolean{pepsQB}{false}}
    
    \ifthenelse{\boolean{pepsQL}}{
        \def\MxB{-2*\l}
        \def\MaNB{north west}
        \def\MaSB{south west}
    }{
        \def\MxB{2*\l}
        \def\MaNB{north east}
        \def\MaSB{south east}
    }
    
    \ifthenelse{\boolean{pepsQB}}{
        \def\MyB{-2*\l}
        \def\MaWB{south west}
        \def\MaEB{south east}
    }{
        \def\MyB{2*\l}
        \def\MaWB{north west}
        \def\MaEB{north east}
    }
    
    \ifthenelse{\boolean{pepsQB}}{
        \node[fake] (g7) at (0,-2*\l) {};
    }{
        \node[fake] (g1) at (0,-\l) {};
    }
    \ifthenelse{\boolean{pepsQT}}{
        \node[fake] (g8) at (0,2*\l) {};
    }{
        \node[fake] (g4) at (0,\l) {};
    }
    \ifthenelse{\boolean{pepsQR}}{
        \node[fake] (g6) at (2*\l,0) {};
    }{
        \node[fake] (g2) at (\l,0) {};
    }
    \ifthenelse{\boolean{pepsQL}}{
        \node[fake] (g5) at (-2*\l,0) {};
    }{
        \node[fake] (g3) at (-\l,0) {};
    }
    
    \ifthenelse{#1=0}{}{
    \fill[color=\cMain] (-\l, -\l) rectangle (\l, \l);
    \ifthenelse{\boolean{pepsQL}}{
        \fill[color=\cQ] (-2*\l, -\l) rectangle (-\l, \l);
    }{}
    \ifthenelse{\boolean{pepsQR}}{
        \fill[color=\cQ] (\l, -\l) rectangle (2*\l, \l);
    }{}
    \ifthenelse{\boolean{pepsQT}}{
        \fill[color=\cQ] (-\l, \l) rectangle (\l, 2*\l);
    }{}
    \ifthenelse{\boolean{pepsQB}}{
        \fill[color=\cQ] (-\l, -2*\l) rectangle (\l, -\l);
    }{}
    }
    
    \node[leg,label={[label distance=-6pt]above left:{${\sss #3}$}}] (f) at (-.25*\l,.25*\l) {};
    
    \ifthenelse{\boolean{pepsQB}}{
        \node[ten,label=right:{${\sss Q_1}$}] (g1) at (0,-\l) {};
    }{
    \ifthenelse{\equal{#6}{v}}{
        \node[ten,label=below:{${\sss #6^{#2}_1}$}] (g1) at (g1) {};
    }{}
    }
    
    \ifthenelse{\boolean{pepsQT}}{
        \node[ten,label=right:{${\sss Q_1}$}] (g4) at (0,\l) {};
    }{
    \ifthenelse{\equal{#9}{\phi}}{
        \node[ten,label=above:{${\sss #9^{#2}_1}$}] (g4) at (g4) {};
    }{}
    }
    
    \ifthenelse{\boolean{pepsQR}}{
        \node[ten,label=below:{${\sss Q_2}$}] (g2) at (\l,0) {};
    }{
    \ifthenelse{\equal{#7}{v}}{
        \node[ten,label=right:{${\sss #7^{#2}_2}$}] (g2) at (g2) {};
    }{}
    }
    
    \ifthenelse{\boolean{pepsQL}}{
        \node[ten,label=below:{${\sss Q_2}$}] (g3) at (-\l,0) {};
    }{
    \ifthenelse{\equal{#8}{\phi}}{
        \node[ten,label=left:{${\sss #8^{#2}_2}$}] (g3) at (g3) {};
    }{}
    }
    
    \node[ten,label={[label distance=-3pt]below left:{${\sss #2}$}}] (n) at (0,0) {};
    
    \draw[obj,->-=.5] (g1) -- (n);
    \draw[obj,->-=.5] (n) -- (g4);
    \draw[obj,->-=.5] (g2) -- (n);
    \draw[obj,->-=.5] (n) -- (g3);
    \ifthenelse{\boolean{pepsQB}}{
        \draw[obj,->-=.5] (g7) -- (g1);
    }{}
    \ifthenelse{\boolean{pepsQT}}{
        \draw[obj,->-=.5] (g4) -- (g8);
    }{}
    \ifthenelse{\boolean{pepsQR}}{
        \draw[obj,->-=.5] (g6) -- (g2);
    }{}
    \ifthenelse{\boolean{pepsQL}}{
        \draw[obj,->-=.5] (g3) -- (g5);
    }{}
    \draw[obj] (n) -- (f);
    
    \ifthenelse{\equal{#4}{}}{}{
        \pepsSplit#4----\pepsEnd
        \let\Mbase\pepsBase
        \pepsCornerLabel{\pepsLi}{pepsQR}{pepsQT}{}{}{north}{east}
        \pepsCornerLabel{\pepsLii}{pepsQR}{pepsQB}{}{-}{south}{east}
        \pepsCornerLabel{\pepsLiii}{pepsQL}{pepsQT}{-}{}{north}{west}
        \pepsCornerLabel{\pepsLiv}{pepsQL}{pepsQB}{-}{-}{south}{west}
    }
    
    \ifthenelse{\equal{#5}{}}{}{
        \pepsSplit#5----\pepsEnd
        \let\MbaseB\pepsBase
        \ifthenelse{\boolean{pepsQL} \or \boolean{pepsQR}}{
        \ifthenelse{\equal{\pepsLi}{-}}{}{
        \node[mlabel, anchor=\MaNB] at (\MxB, \l) {${\sss \MbaseB_{\pepsLi}}$};
    }
    \ifthenelse{\equal{\pepsLii}{-}}{}{
        \node[mlabel, anchor=\MaSB] at (\MxB, -\l) {${\sss \MbaseB_{\pepsLii}}$};
    }
    }{}
    \ifthenelse{\boolean{pepsQT} \or \boolean{pepsQB}}{
    \ifthenelse{\equal{\pepsLi}{-}}{}{
        \node[mlabel, anchor=\MaWB] at (-\l, \MyB) {${\sss \MbaseB_{\pepsLi}}$};
    }
    \ifthenelse{\equal{\pepsLii}{-}}{}{
        \node[mlabel, anchor=\MaEB] at (\l, \MyB) {${\sss \MbaseB_{\pepsLii}}$};
    }
    }{}
    }
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcount\pepscIdx
\def\pepscEndMarker{\pepscEnd}
\def\pepscReset{\advance\pepscIdx by 1 \expandafter\def\csname pepscL\the\pepscIdx\endcsname{-}
    \ifnum\pepscIdx<12 \expandafter\pepscReset\fi}
\def\pepscLoop#1{\def\pepscTmp{#1}
    \ifx\pepscTmp\pepscEndMarker\else
\advance\pepscIdx by 1 \expandafter\let\csname pepscL\the\pepscIdx\endcsname\pepscTmp
\expandafter\pepscLoop
\fi}
\def\pepscSplit#1{\def\pepscBase{#1}\pepscIdx=0 \pepscReset\pepscIdx=0 \pepscLoop}
\newcommand{\pepscLab}[3]{
    \expandafter\let\expandafter\pepscTmpL\csname pepscL#1\endcsname
    \ifthenelse{\equal{\pepscTmpL}{-}}{}{
        \node[mlabel, anchor=#2] at #3 {${\sss \pepscBase_{\pepscTmpL}}$};
    }
}

\newcommand{\PEPSC}[9][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
        \def\l{.75}
        \ifthenelse{\equal{#1}{B}}{
            \def\pepscIn{B}\def\pepscInC{CornflowerBlue!20}
            \def\pepscOut{A}\def\pepscOutC{LimeGreen!20}
        }{
            \def\pepscIn{A}\def\pepscInC{LimeGreen!20}
            \def\pepscOut{B}\def\pepscOutC{CornflowerBlue!20}
        }
        \ifthenelse{\equal{#7}{}}{\def\pepscMode{0}}{
            \ifthenelse{\equal{#7}{Q2Q1}}{\def\pepscMode{3}}{
            \ifthenelse{\equal{#7}{Q1Q2}}{\def\pepscMode{2}}{\def\pepscMode{1}}
            }
        }
        \ifthenelse{\pepscMode=0}{
            \let\pepscX\pepscIn\let\pepscC\pepscInC
        }{
            \let\pepscX\pepscOut\let\pepscC\pepscOutC
        }
        
        \ifthenelse{#2=0}{}{
            \fill[color=\pepscC] (-2*\l, -\l) -- (\l, -\l) -- (\l, 2*\l) -- (-\l, 2*\l) -- (-\l, \l) -- (-2*\l, \l) -- cycle;
            \ifthenelse{\equal{#8}{\phi}}{
                \fill[color=\pepscC] (-3*\l, -\l) rectangle (-2*\l, \l);
                \fill[color=\pepscC] (-\l, 2*\l) rectangle (\l, 3*\l);
            }{}
            \ifthenelse{\pepscMode=1 \or \pepscMode=2}{
                \fill[color=\pepscInC, rounded corners=.4*\l*1cm] (-\l, 0) -- (-.75*\l, .75*\l) [sharp corners] -- (0, \l) -- (\l, \l) -- (\l, -\l) -- (-\l, -\l) -- cycle;
            }{}
            \ifthenelse{\pepscMode=3}{
                \fill[color=\pepscInC] (-\l, -\l) rectangle (\l, \l);
            }{}
        }
        
        \node[leg,label={[label distance=-6pt]above left:{${\sss #3}$}}] (f) at (-.25*\l,.25*\l) {};
        
        \ifthenelse{\equal{#9}{0}}{
            \node[fake] (g1) at (0,-\l) {};
            \node[fake] (g2) at (\l,0) {};
        }{
            \node[ten,label=below:{${\sss v^{\pepscIn}_1}$}] (g1) at (0,-\l) {};
            \node[ten,label=right:{${\sss v^{\pepscIn}_2}$}] (g2) at (\l,0) {};
        }
        \ifthenelse{\pepscMode=2 \or \pepscMode=3}{
            \node[ten,label=below:{${\sss Q_2}$}] (g3) at (-\l,0) {};
            \node[ten,label=right:{${\sss Q_1}$}] (g4) at (0,\l) {};
        }{
        \ifthenelse{\pepscMode=1}{
            \node[ten,draw=none,fill=none,label=below:{${\sss Q_{21}}$}] (g3) at (-\l,0) {};
            \node[ten,draw=none,fill=none] (g4) at (0,\l) {};
        }{}
        }
        \ifthenelse{\equal{#8}{\phi}}{
            \node[ten,label={[label distance=-3pt]below left:{${\sss \pepscX}$}}] (g5) at (-2*\l,0) {};
            \node[ten,label={[label distance=-3pt]below left:{${\sss \pepscX}$}}] (g6) at (0,2*\l) {};
            \node[leg,label={[label distance=-6pt]above left:{${\sss #4}$}}] (f5) at (-2.25*\l,.25*\l) {};
            \node[leg,label={[label distance=-6pt]above left:{${\sss #5}$}}] (f6) at (-.25*\l,2.25*\l) {};
        \ifthenelse{\equal{#9}{0}}{
            \node[fake] (h1) at (-2*\l,-\l) {};
            \node[fake] (h2) at (-2*\l,\l) {};
            \node[fake] (h3) at (-3*\l,0) {};
            \node[fake] (h4) at (-\l,2*\l) {};
            \node[fake] (h5) at (\l,2*\l) {};
            \node[fake] (h6) at (0,3*\l) {};
        }{
            \node[ten,label=below:{${\sss v^{\pepscX}_1}$}] (h1) at (-2*\l,-\l) {};
            \node[ten,label=above:{${\sss \phi^{\pepscX}_1}$}] (h2) at (-2*\l,\l) {};
            \node[ten,label=left:{${\sss \phi^{\pepscX}_2}$}] (h3) at (-3*\l,0) {};
            \node[ten,label=left:{${\sss \phi^{\pepscX}_2}$}] (h4) at (-\l,2*\l) {};
            \node[ten,label=right:{${\sss v^{\pepscX}_2}$}] (h5) at (\l,2*\l) {};
            \node[ten,label=above:{${\sss \phi^{\pepscX}_1}$}] (h6) at (0,3*\l) {};
        }
        }{
            \node[fake] (g5) at (-2*\l,0) {};
            \node[fake] (g6) at (0,2*\l) {};
        }
        
        \node[ten,label={[label distance=-3pt]below left:{${\sss \pepscIn}$}}] (n) at (0,0) {};
        
        \draw[obj,->-=.5] (g1) -- (n);
        \draw[obj,->-=.5] (g2) -- (n);
        \ifthenelse{\pepscMode=0}{
            \draw[obj,->-=.5] (n) -- (g5);
            \draw[obj,->-=.5] (n) -- (g6);
        }{
            \draw[obj,->-=.5] (n) -- (g3);
            \draw[obj,->-=.5] (n) -- (g4);
            \draw[obj,->-=.5] (g3) -- (g5);
            \draw[obj,->-=.5] (g4) -- (g6);
        }
        \ifthenelse{\equal{#8}{\phi}}{
            \draw[obj,->-=.5] (h1) -- (g5);
            \draw[obj,->-=.5] (g5) -- (h2);
            \draw[obj,->-=.5] (g5) -- (h3);
            \draw[obj,->-=.5] (h5) -- (g6);
            \draw[obj,->-=.5] (g6) -- (h4);
            \draw[obj,->-=.5] (g6) -- (h6);
            \draw[obj] (g5) -- (f5);
            \draw[obj] (g6) -- (f6);
        }{}
        \draw[obj] (n) -- (f);
        
        \ifthenelse{\pepscMode=1}{
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round, rounded corners=.4*\l*1cm] (-\l,0) -- (-.75*\l,.75*\l) -- (0,\l);
        }{}
        
        \ifthenelse{\equal{#6}{}}{}{
                \pepscSplit#6\pepscEnd
                \pepscLab{1}{east}{(\l, .5*\l)}
                \pepscLab{2}{south east}{(\l, -\l)}
                \ifthenelse{\pepscMode=1 \or \pepscMode=2}{
                    \pepscLab{3}{center}{(-.5*\l, .65*\l)}
                }{
                \pepscLab{3}{north west}{(-\l, \l)}
            }
                \pepscLab{4}{south}{(-.5*\l, -\l)}
                \ifthenelse{\equal{#8}{\phi}}{
                \pepscLab{5}{east}{(\l, 1.5*\l)}
                \pepscLab{6}{south}{(-1.5*\l, -\l)}
                \pepscLab{7}{north}{(-1.55*\l, \l)}
                \pepscLab{8}{west}{(-\l, 1.55*\l)}
                \pepscLab{9}{north east}{(\l, 3*\l)}
                \pepscLab{10}{north west}{(-\l, 3*\l)}
                \pepscLab{11}{north west}{(-3*\l, \l)}
                \pepscLab{12}{south west}{(-3*\l, -\l)}
            }{
                \pepscLab{5}{north east}{(\l, 2*\l)}
                \pepscLab{6}{south west}{(-2*\l, -\l)}
                \pepscLab{7}{north west}{(-2*\l, \l)}
                \pepscLab{8}{north west}{(-\l, 2*\l)}
            }
        }
    \end{tikzpicture}
}

\newcommand{\PEPSCB}[9][B]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
    \def\l{.75}
        \ifthenelse{\equal{#1}{A}}{
            \def\pepscIn{A}\def\pepscInC{LimeGreen!20}
            \def\pepscOut{B}\def\pepscOutC{CornflowerBlue!20}
        }{
            \def\pepscIn{B}\def\pepscInC{CornflowerBlue!20}
            \def\pepscOut{A}\def\pepscOutC{LimeGreen!20}
        }
        \ifthenelse{\equal{#7}{}}{\def\pepscMode{0}}{
            \ifthenelse{\equal{#7}{Q1Q2}}{\def\pepscMode{3}}{
                \ifthenelse{\equal{#7}{Q1Q2r}}{\def\pepscMode{2}}{\def\pepscMode{1}}
            }
        }
        \ifthenelse{\pepscMode=0}{
            \let\pepscX\pepscIn\let\pepscC\pepscInC
        }{
            \let\pepscX\pepscOut\let\pepscC\pepscOutC
        }
        
        \ifthenelse{#2=0}{}{
            \fill[color=\pepscC] (2*\l, \l) -- (-\l, \l) -- (-\l, -2*\l) -- (\l, -2*\l) -- (\l, -\l) -- (2*\l, -\l) -- cycle;
            \ifthenelse{\equal{#8}{\phi}}{
                \fill[color=\pepscC] (2*\l, -\l) rectangle (3*\l, \l);
                \fill[color=\pepscC] (-\l, -3*\l) rectangle (\l, -2*\l);
            }{}
            \ifthenelse{\pepscMode=1 \or \pepscMode=2}{
                \fill[color=\pepscInC, rounded corners=.4*\l*1cm] (0, -\l) -- (.75*\l, -.75*\l) [sharp corners] -- (\l, 0) -- (\l, \l) -- (-\l, \l) -- (-\l, -\l) -- cycle;
            }{}
            \ifthenelse{\pepscMode=3}{
                \fill[color=\pepscInC] (-\l, -\l) rectangle (\l, \l);
            }{}
        }
        
        \node[leg,label={[label distance=-6pt]above left:{${\sss #3}$}}] (f) at (-.25*\l,.25*\l) {};
        
        \ifthenelse{\equal{#9}{0}}{
            \node[fake] (g3) at (0,\l) {};
            \node[fake] (g4) at (-\l,0) {};
        }{
            \node[ten,label=above:{${\sss \phi^{\pepscIn}_1}$}] (g3) at (0,\l) {};
            \node[ten,label=left:{${\sss \phi^{\pepscIn}_2}$}] (g4) at (-\l,0) {};
        }
        \ifthenelse{\pepscMode=2 \or \pepscMode=3}{
            \node[ten,label=left:{${\sss Q_1}$}] (g1) at (0,-\l) {};
            \node[ten,label=above:{${\sss Q_2}$}] (g2) at (\l,0) {};
        }{
        \ifthenelse{\pepscMode=1}{
            \node[ten,draw=none,fill=none] (g1) at (0,-\l) {};
            \node[ten,draw=none,fill=none,label=above:{${\sss Q_{12}}$}] (g2) at (\l,0) {};
        }{}
        }
        \ifthenelse{\equal{#8}{\phi}}{
            \node[ten,label={[label distance=-3pt]below left:{${\sss \pepscX}$}}] (g5) at (0,-2*\l) {};
            \node[ten,label={[label distance=-3pt]below left:{${\sss \pepscX}$}}] (g6) at (2*\l,0) {};
            \node[leg,label={[label distance=-6pt]above left:{${\sss #5}$}}] (f5) at (-.25*\l,-1.75*\l) {};
            \node[leg,label={[label distance=-6pt]above left:{${\sss #4}$}}] (f6) at (1.75*\l,.25*\l) {};
        \ifthenelse{\equal{#9}{0}}{
            \node[fake] (h1) at (0,-3*\l) {};
            \node[fake] (h2) at (\l,-2*\l) {};
            \node[fake] (h3) at (-\l,-2*\l) {};
            \node[fake] (h4) at (2*\l,-\l) {};
            \node[fake] (h5) at (3*\l,0) {};
            \node[fake] (h6) at (2*\l,\l) {};
        }{
            \node[ten,label=below:{${\sss v^{\pepscX}_1}$}] (h1) at (0,-3*\l) {};
            \node[ten,label=right:{${\sss v^{\pepscX}_2}$}] (h2) at (\l,-2*\l) {};
            \node[ten,label=left:{${\sss \phi^{\pepscX}_2}$}] (h3) at (-\l,-2*\l) {};
            \node[ten,label=below:{${\sss v^{\pepscX}_1}$}] (h4) at (2*\l,-\l) {};
            \node[ten,label=right:{${\sss v^{\pepscX}_2}$}] (h5) at (3*\l,0) {};
            \node[ten,label=above:{${\sss \phi^{\pepscX}_1}$}] (h6) at (2*\l,\l) {};
        }
        }{
            \node[fake] (g5) at (0,-2*\l) {};
            \node[fake] (g6) at (2*\l,0) {};
        }
        
        \node[ten,label={[label distance=-3pt]below left:{${\sss \pepscIn}$}}] (n) at (0,0) {};
        
        \draw[obj,->-=.5] (n) -- (g3);
        \draw[obj,->-=.5] (n) -- (g4);
        \ifthenelse{\pepscMode=0}{
            \draw[obj,->-=.5] (g5) -- (n);
            \draw[obj,->-=.5] (g6) -- (n);
        }{
            \draw[obj,->-=.5] (g1) -- (n);
            \draw[obj,->-=.5] (g2) -- (n);
            \draw[obj,->-=.5] (g5) -- (g1);
            \draw[obj,->-=.5] (g6) -- (g2);
        }
        \ifthenelse{\equal{#8}{\phi}}{
            \draw[obj,->-=.5] (h1) -- (g5);
            \draw[obj,->-=.5] (h2) -- (g5);
            \draw[obj,->-=.5] (g5) -- (h3);
            \draw[obj,->-=.5] (h4) -- (g6);
            \draw[obj,->-=.5] (h5) -- (g6);
            \draw[obj,->-=.5] (g6) -- (h6);
            \draw[obj] (g5) -- (f5);
            \draw[obj] (g6) -- (f6);
        }{}
        \draw[obj] (n) -- (f);
        
        \ifthenelse{\pepscMode=1}{
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round, rounded corners=.4*\l*1cm] (0,-\l) -- (.75*\l,-.75*\l) -- (\l,0);
        }{}
        
        \ifthenelse{\equal{#6}{}}{}{
            \pepscSplit#6\pepscEnd
            \pepscLab{1}{west}{(-\l, -.5*\l)}
            \pepscLab{2}{north west}{(-\l, \l)}
            \ifthenelse{\pepscMode=1 \or \pepscMode=2}{
            \pepscLab{3}{center}{(.38*\l, -.4*\l)}
            }{
                \pepscLab{3}{south east}{(\l, -\l)}
            }
            \pepscLab{4}{north}{(.5*\l, \l)}
            \ifthenelse{\equal{#8}{\phi}}{
            \pepscLab{5}{west}{(-\l, -1.35*\l)}
            \pepscLab{6}{north}{(1.5*\l, \l)}
            \pepscLab{7}{south}{(1.55*\l, -\l)}
            \pepscLab{8}{east}{(\l, -1.55*\l)}
            \pepscLab{9}{south west}{(-\l, -3*\l)}
            \pepscLab{10}{south east}{(\l, -3*\l)}
            \pepscLab{11}{south east}{(3*\l, -\l)}
            \pepscLab{12}{north east}{(3*\l, \l)}
            }{
                \pepscLab{5}{south west}{(-\l, -2*\l)}
                \pepscLab{6}{north east}{(2*\l, \l)}
                \pepscLab{7}{south east}{(2*\l, -\l)}
                \pepscLab{8}{south east}{(\l, -2*\l)}
            }
        }
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcommand{\QTTLine}[7][1]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,.5*.75)}, mlabel/.style={inner sep=1pt}]
        \def\l{.75}
        \IfEndWith{#2}{a}{\def\qqSplit{a}}{\IfEndWith{#2}{b}{\def\qqSplit{b}}{\def\qqSplit{}}}
        \ifthenelse{#1=0}{}{
            \ifthenelse{\equal{\qqSplit}{a}}{
                \fill[color=CornflowerBlue!20] (-\l, -\l) rectangle (\l, 2*\l);
                \fill[color=LimeGreen!20] (0, -\l) rectangle (\l, .45*\l);
                \fill[color=LimeGreen!20] (0, .55*\l) rectangle (\l, 2*\l);
                \fill[white] (\l, .5*\l) circle (.12*\l);
            }{
            \ifthenelse{\equal{\qqSplit}{b}}{
                \fill[color=LimeGreen!20] (-\l, -\l) rectangle (\l, 2*\l);
                \fill[color=CornflowerBlue!20] (-\l, -\l) rectangle (0, .45*\l);
                \fill[color=CornflowerBlue!20] (-\l, .55*\l) rectangle (0, 2*\l);
                \fill[white] (-\l, .5*\l) circle (.12*\l);
            }{
                \fill[color=LimeGreen!20] (0, -\l) rectangle (\l, 2*\l);
                \fill[color=CornflowerBlue!20] (-\l, -\l) rectangle (0, 2*\l);
            }
            }
        }
        \ifthenelse{\equal{#4}{}}{
            \node[fake] (a0) at (\l,0) {};
        }{
            \node[ten,label=right:{${\sss #4}$}] (a0) at (\l,0) {};
        }
        \ifthenelse{\equal{#5}{}}{
            \node[fake] (a1) at (\l,\l) {};
        }{
            \node[ten,label=right:{${\sss #5}$}] (a1) at (\l,\l) {};
        }
        \ifthenelse{\equal{#6}{}}{
            \node[fake] (b0) at (-\l,0) {};
        }{
            \node[ten,label=left:{${\sss #6}$}] (b0) at (-\l,0) {};
        }
        \ifthenelse{\equal{#7}{}}{
            \node[fake] (b1) at (-\l,\l) {};
        }{
            \node[ten,label=left:{${\sss #7}$}] (b1) at (-\l,\l) {};
        }
        \IfBeginWith{#2}{Q1Q2}{\def\qqSep{1}}{\IfBeginWith{#2}{Q2Q1}{\def\qqSep{1}}{\def\qqSep{0}}}
        \ifthenelse{\qqSep=1}{
            \IfBeginWith{#2}{Q1Q2}{\def\qqLow{Q_1}\def\qqUp{Q_2}}{\def\qqLow{Q_2}\def\qqUp{Q_1}}
            \node[ten,label=below:{${\sss \qqLow}$}] (q0) at (0,0) {};
            \node[ten,label=above:{${\sss \qqUp}$}] (q1) at (0,\l) {};
        }{
        \ifthenelse{\equal{#2}{Q12}}{\def\qqBand{Q_{12}}}{\def\qqBand{Q_{21}}}
            \node[ten,draw=none,fill=none,label=below:{${\sss \qqBand}$}] (q0) at (0,0) {};
            \node[ten,draw=none,fill=none] (q1) at (0,\l) {};
        }
        \draw[obj,->-=.55] (a0) -- (q0);
        \draw[obj,->-=.6] (q0) -- (b0);
        \draw[obj,->-=.55] (a1) -- (q1);
        \draw[obj,->-=.6] (q1) -- (b1);
        \ifthenelse{\qqSep=1}{}{
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round] (0,0) -- (0,\l);
        }
        \ifthenelse{\equal{#3}{}}{}{
            \pepscSplit#3\pepscEnd
            \pepscLab{1}{north east}{(\l, 2*\l)}
            \pepscLab{2}{east}{(\l, .5*\l)}
            \pepscLab{3}{south east}{(\l, -\l)}
            \pepscLab{4}{north west}{(-\l, 2*\l)}
            \pepscLab{5}{west}{(-\l, .5*\l)}
            \pepscLab{6}{south west}{(-\l, -\l)}
            \ifthenelse{\equal{\qqSplit}{a}}{
                \pepscLab{7}{north east}{(\l, .44*\l)}
                \pepscLab{8}{south east}{(\l, .56*\l)}
            }{}
            \ifthenelse{\equal{\qqSplit}{b}}{
                \pepscLab{7}{north west}{(-\l, .44*\l)}
                \pepscLab{8}{south west}{(-\l, .56*\l)}
            }{}
        }
    \end{tikzpicture}
}

\newcommand{\QSQ}[6][1]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}, mlabel/.style={inner sep=1pt}]
        \def\l{.75}
        \ifthenelse{\equal{#2}{Q1}}{\def\qsqLab{Q_1}}{\ifthenelse{\equal{#2}{Q2}}{\def\qsqLab{Q_2}}{\def\qsqLab{#2}}}
        \ifthenelse{#1=0}{}{
            \fill[color=LimeGreen!20] (0, -\l) rectangle (\l, \l);
            \fill[color=CornflowerBlue!20] (-\l, -\l) rectangle (0, \l);
        }
        \node[fake] (a) at (\l,0) {};
        \node[fake] (b) at (-\l,0) {};
        \node[ten,label=below:{${\sss \qsqLab}$}] (q) at (0,0) {};
        \draw[obj,->-=.55] (a) -- (q);
        \draw[obj,->-=.6] (q) -- (b);
        \ifthenelse{\equal{#3}{}}{}{\node[mlabel, anchor=north east] at (\l, \l) {${\sss #3}$};}
        \ifthenelse{\equal{#4}{}}{}{\node[mlabel, anchor=south east] at (\l, -\l) {${\sss #4}$};}
        \ifthenelse{\equal{#5}{}}{}{\node[mlabel, anchor=north west] at (-\l, \l) {${\sss #5}$};}
        \ifthenelse{\equal{#6}{}}{}{\node[mlabel, anchor=south west] at (-\l, -\l) {${\sss #6}$};}
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcommand{\PEPSQ}[8][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,-.75)}, mlabel/.style={inner sep=1pt}]
        \def\l{.75}
        \ifthenelse{\equal{#6}{} \and \equal{#7}{}}{
            \ifthenelse{\equal{#1}{B}}{\def\pqF{B}\def\pqFC{CornflowerBlue!20}}{\def\pqF{A}\def\pqFC{LimeGreen!20}}
            \let\pqC\pqF\let\pqCC\pqFC
        }{
            \def\pqF{A}\def\pqFC{LimeGreen!20}
            \ifthenelse{\equal{#7}{} \and \not\equal{#6}{Q21}}{\def\pqC{A}\def\pqCC{LimeGreen!20}}{\def\pqC{B}\def\pqCC{CornflowerBlue!20}}
        }
        \def\pqOutCoup{0}\def\pqMidCoup{0}
        \ifthenelse{\equal{#6}{Q} \or \equal{#6}{Qr}}{\def\pqOutCoup{1}\def\pqMidCoup{1}}{}
        \ifthenelse{\equal{#6}{QQ}}{\def\pqOutCoup{1}}{}
        
        \ifthenelse{#2=0}{}{
            \ifthenelse{\equal{#6}{}}{\def\pqBG{\pqCC}}{\def\pqBG{CornflowerBlue!20}}
            \fill[color=\pqBG] (-2*\l, -3*\l) -- (\l, -3*\l) -- (\l, -\l) -- (3*\l, -\l) -- (3*\l, 2*\l) -- (-\l, 2*\l) -- (-\l, \l) -- (-2*\l, \l) -- cycle;
            \ifthenelse{\equal{#6}{Q21}}{
                \fill[color=\pqFC, rounded corners=.4*\l*1cm] (-\l, -2*\l) -- (-.75*\l, -1.25*\l) [sharp corners] -- (0, -\l) -- (\l, -\l) -- (\l, -3*\l) -- (-\l, -3*\l) -- cycle;
                \fill[color=\pqFC, rounded corners=.4*\l*1cm] (\l, 0) -- (1.25*\l, .75*\l) [sharp corners] -- (2*\l, \l) -- (3*\l, \l) -- (3*\l, -\l) -- (\l, -\l) -- cycle;
            }{
                \ifthenelse{\equal{#6}{}}{
                    \ifthenelse{\equal{#7}{}}{}{
                        \fill[color=\pqFC] (-2*\l, -3*\l) rectangle (\l, -\l);
                        \fill[color=\pqFC] (\l, -\l) rectangle (3*\l, 2*\l);
                    }
                }{
                    \ifthenelse{\equal{#7}{}}{
                        \ifthenelse{\equal{#6}{Q2211} \or \equal{#6}{Qr}}{
                            \fill[color=\pqFC, rounded corners=.4*\l*1cm] (-\l, 0) -- (-.75*\l, .75*\l) [sharp corners] -- (0, \l) -- (3*\l, \l) -- (3*\l, -\l) -- (\l, -\l) -- (\l, -3*\l) -- (-\l, -3*\l) -- cycle;
                        }{
                            \fill[color=\pqFC] (-\l, -3*\l) -- (\l, -3*\l) -- (\l, -\l) -- (3*\l, -\l) -- (3*\l, \l) -- (-\l, \l) -- cycle;
                        }
                    }{
                        \fill[color=\pqFC] (-\l, -3*\l) rectangle (\l, -\l);
                        \fill[color=\pqFC] (\l, -\l) rectangle (3*\l, \l);
                    }
                }
            }
            \ifthenelse{\equal{#7}{}}{}{
                \ifthenelse{\equal{#7}{Q12} \or \equal{#7}{Q1Q2r}}{
                    \fill[color=\pqFC] (0, -\l) rectangle (\l, 0);
                    \fill[color=\pqCC, rounded corners=.4*\l*1cm] (0, -\l) -- (.75*\l, -.75*\l) [sharp corners] -- (\l, 0) -- (\l, \l) -- (-\l, \l) -- (-\l, -\l) -- cycle;
                }{
                    \fill[color=\pqCC] (-\l, -\l) rectangle (\l, \l);
                }
            }
        }
        
        \node[leg,label={[label distance=-6pt]above left:{${\sss #3}$}}] (f) at (-.25*\l,.25*\l) {};
        \node[leg,label={[label distance=-6pt]above left:{${\sss #5}$}}] (fS) at (-.25*\l,-1.75*\l) {};
        \node[leg,label={[label distance=-6pt]above left:{${\sss #4}$}}] (fE) at (1.75*\l,.25*\l) {};
        
        \ifthenelse{\equal{#8}{0}}{
            \node[fake] (s1) at (0,-3*\l) {};
            \node[fake] (s2) at (\l,-2*\l) {};
            \node[fake] (e1) at (2*\l,-\l) {};
            \node[fake] (e2) at (3*\l,0) {};
        }{
            \node[ten,label=below:{${\sss v^{\pqF}_1}$}] (s1) at (0,-3*\l) {};
            \node[ten,label=right:{${\sss v^{\pqF}_2}$}] (s2) at (\l,-2*\l) {};
            \node[ten,label=below:{${\sss v^{\pqF}_1}$}] (e1) at (2*\l,-\l) {};
            \node[ten,label=right:{${\sss v^{\pqF}_2}$}] (e2) at (3*\l,0) {};
        }
        
        \ifthenelse{\equal{#6}{Q21}}{
            \node[ten,draw=none,fill=none] (i1) at (0,-\l) {};
            \node[ten,draw=none,fill=none,label=below:{${\sss Q_{21}}$}] (i2) at (\l,0) {};
        }{}
            \ifthenelse{\equal{#7}{Q1Q2} \or \equal{#7}{Q1Q2r}}{
            \node[ten,label=left:{${\sss Q_1}$}] (i1) at (0,-\l) {};
            \node[ten,label=above:{${\sss Q_2}$}] (i2) at (\l,0) {};
        }{
            \ifthenelse{\equal{#7}{Q12}}{
                \node[ten,draw=none,fill=none] (i1) at (0,-\l) {};
                \node[ten,draw=none,fill=none,label=above:{${\sss Q_{12}}$}] (i2) at (\l,0) {};
            }{}
        }
        \node[fake] (p1) at (-2*\l,-2*\l) {};
        \node[fake] (p2) at (-2*\l,0) {};
        \node[fake] (p3) at (0,2*\l) {};
        \node[fake] (p4) at (2*\l,2*\l) {};
        \ifthenelse{\equal{#6}{Q21}}{
            \node[ten,draw=none,fill=none,label=below:{${\sss Q_{21}}$}] (o1) at (-\l,-2*\l) {};
            \node[ten,draw=none,fill=none] (o4) at (2*\l,\l) {};
        }{}
        \ifthenelse{\equal{#6}{Q2211}}{
            \node[ten,draw=none,fill=none] (o1) at (-\l,-2*\l) {};
            \node[ten,draw=none,fill=none] (o2) at (-\l,0) {};
            \node[ten,draw=none,fill=none] (o3) at (0,\l) {};
            \node[ten,draw=none,fill=none] (o4) at (2*\l,\l) {};
        }{
        \ifthenelse{\pqOutCoup=1}{
            \node[ten,label=below:{${\sss Q_2}$}] (o1) at (-\l,-2*\l) {};
            \node[ten,label=right:{${\sss Q_1}$}] (o4) at (2*\l,\l) {};
        }{}
        \ifthenelse{\pqMidCoup=1}{
            \node[ten,label=below:{${\sss Q_2}$}] (o2) at (-\l,0) {};
            \node[ten,label=right:{${\sss Q_1}$}] (o3) at (0,\l) {};
        }{}
        }
        
        \node[ten,label={[label distance=-3pt]below left:{${\sss \pqC}$}}] (n) at (0,0) {};
        \node[ten,label={[label distance=-3pt]below left:{${\sss \pqF}$}}] (S) at (0,-2*\l) {};
        \node[ten,label={[label distance=-3pt]below left:{${\sss \pqF}$}}] (E) at (2*\l,0) {};
        
        \draw[obj,->-=.5] (s1) -- (S);
        \draw[obj,->-=.5] (s2) -- (S);
        \draw[obj,->-=.5] (e1) -- (E);
        \draw[obj,->-=.5] (e2) -- (E);
        \ifthenelse{\equal{#7}{} \and \not\equal{#6}{Q21}}{
            \draw[obj,->-=.5] (S) -- (n);
            \draw[obj,->-=.5] (E) -- (n);
        }{
            \draw[obj,->-=.5] (S) -- (i1);
            \draw[obj,->-=.5] (i1) -- (n);
            \draw[obj,->-=.5] (E) -- (i2);
            \draw[obj,->-=.5] (i2) -- (n);
        }
        \ifthenelse{\equal{#6}{Q2211} \or \equal{#6}{Q21} \or \pqOutCoup=1}{
            \draw[obj,->-=.5] (S) -- (o1);
            \draw[obj,->-=.5] (o1) -- (p1);
            \draw[obj,->-=.5] (E) -- (o4);
            \draw[obj,->-=.5] (o4) -- (p4);
        }{
            \draw[obj,->-=.5] (S) -- (p1);
            \draw[obj,->-=.5] (E) -- (p4);
        }
        \ifthenelse{\equal{#6}{Q2211} \or \pqMidCoup=1}{
            \draw[obj,->-=.5] (n) -- (o2);
            \draw[obj,->-=.5] (o2) -- (p2);
            \draw[obj,->-=.5] (n) -- (o3);
            \draw[obj,->-=.5] (o3) -- (p3);
        }{
            \draw[obj,->-=.5] (n) -- (p2);
            \draw[obj,->-=.5] (n) -- (p3);
        }
        \draw[obj] (n) -- (f);
        \draw[obj] (S) -- (fS);
        \draw[obj] (E) -- (fE);
        
        \ifthenelse{\equal{#7}{Q12}}{
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round, rounded corners=.4*\l*1cm] (0,-\l) -- (.75*\l,-.75*\l) -- (\l,0);
        }{}
        \ifthenelse{\equal{#6}{Q21}}{
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round, rounded corners=.4*\l*1cm] (-\l,-2*\l) -- (-.75*\l,-1.25*\l) -- (0,-\l);
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round, rounded corners=.4*\l*1cm] (\l,0) -- (1.25*\l,.75*\l) -- (2*\l,\l);
        }{}
        \ifthenelse{\equal{#6}{Q2211}}{
            \draw[double=gray!20, double distance=\dimexpr4.3pt-\pgflinewidth\relax, line cap=round] (-\l,-2*\l) [rounded corners=.2*\l*1cm] -- (-\l,0) [rounded corners=.4*\l*1cm] -- (-.75*\l,.75*\l) [rounded corners=.2*\l*1cm] -- (0,\l) -- (2*\l,\l);
            \node[mlabel, anchor=east] at (-1.1*\l, -\l) {${\sss Q_{2211}}$};
        }{}
    \end{tikzpicture}
}

% ------------------------------------------------------

\newcommand{\PEPSord}[2][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (-\l,0) -- (\l,0);
        \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (0,-\l) -- (0,\l);
        \node[leg,label={[label distance=-6pt]above left:{${\sss #2}$}}] (f) at (-.25*\l,.25*\l) {};
        \node[fake] (g1) at (0,-\l) {};
        \node[fake] (g2) at (\l,0) {};
        \node[fake] (g3) at (-\l,0) {};
        \node[fake] (g4) at (0,\l) {};
        \node[ten,label={[label distance=-3pt]below left:{${\sss #1}$}}] (n) at (0,0) {};
        \draw[obj,->-=.5] (g1) -- (n);
        \draw[obj,->-=.5] (n) -- (g4);
        \draw[obj,->-=.5] (g2) -- (n);
        \draw[obj,->-=.5] (n) -- (g3);
        \draw[obj] (n) -- (f);
    \end{tikzpicture}
}
\newcommand{\PEPSmps}[2][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \draw[LimeGreen!50,line width=1.2pt] (-\l,-\l) -- (0,-\l) to[bend right=45] (\l,0) -- (\l,\l);
        \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (-\l,0) -- (\l,0);
        \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (0,-\l) -- (0,\l);
        \node[leg,label={[label distance=-6pt]above left:{${\sss #2}$}}] (f) at (-.25*\l,.25*\l) {};
        \node[ten,label=below:{${\sss v^{#1}_1}$}] (g1) at (0,-\l) {};
        \node[ten,label=right:{${\sss v^{#1}_2}$}] (g2) at (\l,0) {};
        \node[fake] (g3) at (-\l,0) {};
        \node[fake] (g4) at (0,\l) {};
        \node[ten,label={[label distance=-3pt]below left:{${\sss #1}$}}] (n) at (0,0) {};
        \draw[obj,->-=.5] (g1) -- (n);
        \draw[obj,->-=.5] (n) -- (g4);
        \draw[obj,->-=.5] (g2) -- (n);
        \draw[obj,->-=.5] (n) -- (g3);
        \draw[obj] (n) -- (f);
    \end{tikzpicture}
}

\newcommand{\PEPSmpsco}[2][A]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \draw[LimeGreen!50,line width=1.2pt] (-\l,-\l) -- (-\l,0) to[bend left=45] (0,\l) -- (\l,\l);
        \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (-\l,0) -- (\l,0);
        \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (0,-\l) -- (0,\l);
        \node[leg,label={[label distance=-6pt]above left:{${\sss #2}$}}] (f) at (-.25*\l,.25*\l) {};
        \node[fake] (g1) at (0,-\l) {};
        \node[fake] (g2) at (\l,0) {};
        \node[ten,label=left:{${\sss \phi^{#1}_2}$}] (g3) at (-\l,0) {};
        \node[ten,label=above:{${\sss \phi^{#1}_1}$}] (g4) at (0,\l) {};
        \node[ten,label={[label distance=-3pt]below left:{${\sss #1}$}}] (n) at (0,0) {};
        \draw[obj,->-=.5] (g1) -- (n);
        \draw[obj,->-=.5] (n) -- (g4);
        \draw[obj,->-=.5] (g2) -- (n);
        \draw[obj,->-=.5] (n) -- (g3);
        \draw[obj] (n) -- (f);
    \end{tikzpicture}
}

\newcommand{\PEPSQord}[2]{
    \begin{tikzpicture}[baseline={([yshift=-.6ex]0,0)}]
        \def\l{.75}
        \ifthenelse{\equal{#1}{21}}{
            \draw[CornflowerBlue!50,line width=2.4pt,line cap=butt] (-\l,-\l) -- (-\l,0) to[bend left=45] (0,\l) -- (\l,\l);
            \begin{scope}
                \clip (-\l,-\l) -- (-\l,0) to[bend left=45] (0,\l) -- (\l,\l) -- (\l,-\l) -- cycle;
                \draw[LimeGreen!50,line width=2.4pt,line cap=butt] (-\l,-\l) -- (-\l,0) to[bend left=45] (0,\l) -- (\l,\l);
            \end{scope}
            \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (\l,0) -- (-\l,0);
            \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (0,-\l) -- (0,\l);
            \draw[CornflowerBlue!50,line width=2.6pt,line cap=butt] (-\l,0) -- (-2*\l,0);
            \draw[CornflowerBlue!50,line width=2.6pt,line cap=butt] (0,\l) -- (0,2*\l);
            \node[fake] (g1) at (0,-\l) {};
            \node[fake] (g2) at (\l,0) {};
            \node[ten,label=below left:{${\sss Q_2}$}] (q2) at (-\l,0) {};
            \node[ten,label=above right:{${\sss Q_1}$}] (q1) at (0,\l) {};
            \node[fake] (g3) at (-2*\l,0) {};
            \node[fake] (g4) at (0,2*\l) {};
            \node[leg,label={[label distance=-6pt]above left:{${\sss #2}$}}] (f) at (-.25*\l,.25*\l) {};
            \node[ten,label={[label distance=-3pt]below left:{${\sss A}$}}] (n) at (0,0) {};
            \draw[obj,->-=.5] (g1) -- (n);
            \draw[obj,->-=.5] (g2) -- (n);
            \draw[obj,->-=.5] (n) -- (q2);
            \draw[obj,->-=.5] (n) -- (q1);
            \draw[obj,->-=.5] (q2) -- (g3);
            \draw[obj,->-=.5] (q1) -- (g4);
            \draw[obj] (n) -- (f);
        }{
            \draw[LimeGreen!50,line width=2.4pt,line cap=butt] (-\l,-\l) -- (0,-\l) to[bend right=45] (\l,0) -- (\l,\l);
            \begin{scope}
                \clip (-\l,-\l) -- (0,-\l) to[bend right=45] (\l,0) -- (\l,\l) -- (-\l,\l) -- cycle;
                \draw[CornflowerBlue!50,line width=2.4pt,line cap=butt] (-\l,-\l) -- (0,-\l) to[bend right=45] (\l,0) -- (\l,\l);
            \end{scope}
            \draw[CornflowerBlue!50,line width=2.6pt,line cap=butt] (\l,0) -- (-\l,0);
            \draw[CornflowerBlue!50,line width=2.6pt,line cap=butt] (0,-\l) -- (0,\l);
            \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (\l,0) -- (2*\l,0);
            \draw[LimeGreen!50,line width=2.6pt,line cap=butt] (0,-\l) -- (0,-2*\l);
            \node[fake] (g1) at (0,-2*\l) {};
            \node[fake] (g2) at (2*\l,0) {};
            \node[ten,label=below left:{${\sss Q_1}$}] (q1) at (0,-\l) {};
            \node[ten,label=above right:{${\sss Q_2}$}] (q2) at (\l,0) {};
            \node[fake] (g3) at (-\l,0) {};
            \node[fake] (g4) at (0,\l) {};
            \node[leg,label={[label distance=-6pt]above left:{${\sss #2}$}}] (f) at (-.25*\l,.25*\l) {};
            \node[ten,label={[label distance=-3pt]below left:{${\sss B}$}}] (n) at (0,0) {};
            \draw[obj,->-=.5] (g1) -- (q1);
            \draw[obj,->-=.5] (g2) -- (q2);
            \draw[obj,->-=.5] (q1) -- (n);
            \draw[obj,->-=.5] (q2) -- (n);
            \draw[obj,->-=.5] (n) -- (g3);
            \draw[obj,->-=.5] (n) -- (g4);
            \draw[obj] (n) -- (f);
        }
    \end{tikzpicture}
}
